Zero-Shot Verification-guided Chain of Thoughts

Previous works have demonstrated the effectiveness of Chain-of-Thought (COT) prompts and verifiers in guiding Large Language Models (LLMs) through the space of reasoning. However, most such studies either use a fine-tuned verifier or rely on manually handcrafted few-shot examples. In contrast, in this paper, we focus on LLM-based self-verification of self-generated reasoning steps via COT prompts in a completely zero-shot regime. To explore this setting, we design a new zero-shot prompt, which we call COT STEP, to aid zero-shot decomposition of reasoning steps and design two new zero-shot prompts for LLM-based verifiers. We evaluate the verifiers' ability to classify the correctness of reasoning chains and explore different ways to use verifier scores in guiding reasoning for various mathematical and commonsense reasoning tasks with different LLMs.

==> introduction.tex <==
\section{Introduction}
\label{sec:intro}
% \looseness=-2
Transformer \cite{vaswani2017attention} is a highly successful general-purpose attention-based architecture that aims to eliminate any recurrence or convolution. Nevertheless, several works have questioned whether the complete elimination of recurrence has been the right move \cite{han2021transformer,hao2022formal,merrill2022saturated}. Although Transformers generally perform better than Recurrent Neural Networks (RNNs) given enough data,\footnote{Newer RNNs like RWKV \cite{peng2023rwkv} or Mamba \cite{gu2024mamba} could be potential exceptions.} several works have shown that RNNs can still outperform Transformers in specific contexts - especially in algorithmic and structure-sensitive tasks under out-of-distribution (OOD) settings \cite{tran2018importance,han2021transformer,shen2019ordered,bhattamishra2023simplicity,liu2023exposing,deletang2023neural}. Theoretical reasons \cite{han2021transformer,hao2022formal,merrill2022saturated} are also suggested for such limitations of Transformers. Overall, these factors naturally raise the question of whether we can get ``the best of both worlds'' by combining recurrence and Transformers in the same model. % in some fashion.

As a motivating example, consider a task like ListOps \cite{nangia2018listops} where we have to solve a nested list of mathematical operations such as: 
{\small{\verb+MAX(1,3,SUM(4,5,MIN(9,7)),4))+}}. Note that in such a task, unconstrained all-to-all (all tokens to all tokens) interactions cannot accommodate for fixed layer depth in Transformers \cite{vaswani2017attention} compared to RNNs where layer depth can extend adaptively based on sequence length. To solve this task, a model has to process the sequence sequentially because the operations in the outer lists can only be executed once the inner list operations are executed. Keeping that in mind, we can list a few potentially necessary {\em conditions} or requirements to fulfill for a task like this (and other tasks like program synthesis, program execution, mathematical reasoning, algorithmic reasoning, etc.):\footnote{A similar list of requirements was also motivated in \citet{csordas2022the}.}

\begin{itemize}
    \item \textbf{C1: }Ability to operate in arbitrary orders (for example, the innermost operations may occur in any position in the input). 
    \item \textbf{C2: } Being equipped with a gating mechanism to keep some hidden states unchanged if needed (for example, outermost values may need to remain unchanged for a while to wait for inner list operations to be completed). 
    \item \textbf{C3: } Having adaptive number of layers (according to the input) such that the number of layers can potentially increase indefinitely with higher demand (for example, when a higher depth of reasoning is required according to sequence length as longer sequences are more complex).%\footnote{Other alternatives besides increasing depth-wise layer can be to use scratchpad \cite{nye2021show} or induce chain of thought reasoning \cite{wei2022chain} to offload some intermediate computation horizontally in the temporal direction.}.
\end{itemize}

Transformers \cite{vaswani2017attention} with their fixed layers (failing C3) and lacking a gating mechanism to control information flow (failing C2) tend to struggle in tasks like ListOps \cite{tran2018importance,shen2019ordered,tay2021long,csordas2022the} especially in out-of-distribution contexts - for example, when evaluated on data of higher sequence length compared to the length of training samples. \citet{zhou2023algorithms} show that standard Transformers are most suited for length generalization when the problem can be solved by a short RASP-L program; failing otherwise - such as by learning spurious shortcuts \cite{liu2023transformers}. 

Given these issues, we consider two broad directions of including recurrence in Transformers to tackle these limitations---one via adding depth-wise recurrence ($\S$\ref{sec:depthwise}, $\S$\ref{sec:p-depthwise}) and another via adding chunk-wise recurrence ($\S$\ref{sec:chunkwise}, $\S$\ref{sec:p-chunkwise}).

\noindent  \textbf{1. Depth-wise Recurrence:} One way to introduce recurrence is to {\em repeat the same Transformer block over all tokens}. Such a strategy is employed by Universal Transformer (UT) \cite{dehghani2018universal}. In the complete implementation, this is accompanied by a dynamic halting mechanism \cite{graves2016adaptive} that adaptively decides when to halt based on the input complexity. We consider Universal Transformer with a modern variant of its halting function \cite{tan2023sparse} as the representative model to study for this direction (baseline UT). We present more related works on depth-wise recurrence and dynamic halting in Appendix \ref{sec:related works}. 

\noindent  \textbf{2. Chunk-wise Recurrence:} Another way to introduce recurrence is to {\em incorporate temporal recurrence just like RNNs do} except with a stack of Transformer blocks as the recurrent cell, using the past hidden states or some compressed representation as the internal RNN-like memory \cite{fan2020addressing}. Typically, this temporal recurrence is done at the level of chunks (subsequences) rather than single tokens to exploit the parallelism of Transformers \cite{didolkar2022temporal, ju2022staircase, hutchins2022blockrecurrent, bulatov2022recurrent}. In other words, these models can recurrently process one whole chunk at a time rather than single tokens during training. We consider Temporal Latent Bottleneck (TLB) \cite{didolkar2022temporal} as the representative model to study for this direction (baseline TLB). 

Chunk-wise recurrence can also be backed by some practical engineering-related motivations. For example, Transformer XL \cite{dai2019transformer} enables a recurrent cache mechanism to compress past information into a fixed number of memory slots for efficient language modeling. This bypasses the need for expensive attention to an indefinitely growing history of tokens. Other methods have extended this strategy with gradient propagation through the memory slots for long-range language modeling \cite{hutchins2022blockrecurrent,ju2022staircase,bulatov2022recurrent,hwang2024transformerfam}. Some recent works have suggested that recurrent augmentation provides better memory for Transformers \cite{kuratov2024search,bulatov2024beyond}.

%Both forms of recurrence can help Transformers dynamically adapt to input complexity \cite{graves2016adaptive} - for example, dynamically increase or decrease the layers assigned to an input based on its complexity. One way to achieve this is to use a recurrent application of a layer with an input-dependent dynamic halting mechanism. Recurrence can, in principle, allow the model to assign an unbounded amount of layers depending on the task complexity \cite{dehghani2018universal,tan2023sparse,banino2021ponder}.

\vspace{1mm}
\noindent  \textbf{Contributions:} We propose Gated Universal Transformer (GUT) that uses a transition-aware global dynamic halting mechanism for Universal Transformer and integrates it with a gating mechanism and transition-dynamics-aware halting function. We also propose Gated Universal Transformer Latent Bottleneck (GUTLB) as a combination of GUT (Depth-wise Recurrent Transformer) with TLB (Chunk-wise Recurrent Transformer). We comprehensively investigate the advantages and disadvantages of the two forms of recurrences and our modifications in several diagnostic tasks such as Long Range Arena (LRA), flip-flop language modeling, ListOps, and Logical Inference.

We find that GUT tends to perform better than baseline UT in most of the algorithmic tasks tested here, but so far, we have not found much advantage for using GUTLB over TLB. We also show that chunk-wise recurrence with its fixed recurrent attention window tends to show more robustness than depth-wise recurrence in length generalization and flip-flop language modeling but worse IID performance in certain structure-sensitive tasks like ListOps and logical inference.
